CNN Image Retrieval Learns from BoW: Unsupervised Fine-Tuning with Hard Examples

Convolutional Neural Networks (CNNs) achieve state-of-the-art performance in many computer vision tasks. However, this achievement is preceded by extreme manual annotation in order to perform either training from scratch or fine-tuning for the target task. In this work, we propose to fine-tune CNN for image retrieval from a large collection of unordered images in a fully automated manner. We employ state-of-the-art retrieval and Structure-from-Motion (SfM) methods to obtain 3D models, which are used to guide the selection of the training data for CNN fine-tuning. We show that both hard positive and hard negative examples enhance the final performance in particular object retrieval with compact codes.

==> no-plots.tex <==
\newcommand{\extfig}[2]{!}
\newcommand{\extdata}[1]{}


==> plots.tex <==
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{pgf,tikz}


%------------------------------------------------------------------------------
\usepgfplotslibrary{external}
\tikzexternalize
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\extdata}[1]{\input{#1}}
%------------------------------------------------------------------------------

\newcommand{\leg}[1]{\addlegendentry{#1}}

